SoK: Rethinking Membership Inference in Tabular Machine Learning

Membership Inference Attacks (MIAs) are currently the dominant approach to evaluating privacy in machine learning applications. Despite their significance, several concerns remain unexplored, particularly with regard to tabular data. Existing evaluations focus predominantly on high-dimensional datasets, leaving the privacy behavior of small-to-medium datasets unexplored. In this paper, we present a new taxonomy for MIAs and conduct a comprehensive study of the factors influencing vulnerability. We evaluate four distinct state-of-the-art attacks across diverse tabular datasets and model architectures. Our results show that datasets with higher class granularity and majority class percentage are more susceptible to MIAs. We further demonstrate that advanced MIAs are highly dependent on adversarial knowledge of the target model, while reference model-free attacks often achieve statistically comparable results. Most importantly, we show that records with unique signatures (single-outs) remain highly vulnerable, even when common defenses are applied. These findings indicate that current defenses reduce average leakage, but fail to adequately protect the most sensitive individuals.

==> tables/dp-smote.tex <==
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llccccccccc}
\toprule
& & \multicolumn{3}{c}{COMPAS} & \multicolumn{3}{c}{Surgery} & \multicolumn{3}{c}{MIC} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
Attack & Model & 0.01 & 0.5 & 1 & 0.01 & 0.5 & 1 & 0.01 & 0.5 & 1 \\
\midrule
\multirow{3}{*}{RMIA} & MLP & -0.6 & -0.5 & +2.0 & -12.3 & +1.8 & -5.8 & -14.7 & +44.5 & +32.6 \\
 & RF & -0.7 & -0.1 & -2.9 & -13.8 & -10.5 & -10.1 & -4.7 & +35.0 & +36.2 \\
 & LR & +1.0 & +0.7 & +0.8 & -0.9 & -0.4 & -0.1 & +2.4 & -3.0 & -3.5 \\
\midrule
\multirow{3}{*}{LiRA} & MLP & +3.8 & +3.8 & +5.4 & +0.7 & +11.8 & +4.4 & -6.1 & +26.8 & +21.1 \\
 & RF & -1.3 & -0.2 & -2.1 & -2.8 & -0.8 & -0.7 & -0.6 & +16.9 & +17.8 \\
 & LR & +1.2 & +0.8 & +0.4 & -1.0 & -0.0 & +0.2 & +5.2 & +5.5 & +4.6 \\
\midrule
\multirow{3}{*}{Attack-P} & MLP & +6.8 & +5.2 & +8.5 & +5.2 & +17.1 & +13.1 & -1.8 & +55.4 & +39.1 \\
 & RF & -0.5 & -0.4 & -1.8 & +6.7 & +8.7 & +8.9 & -0.4 & +24.4 & +27.2 \\
 & LR & +0.7 & +0.3 & +0.3 & +2.3 & +0.9 & +0.7 & +21.1 & +4.8 & +3.3 \\
\midrule
\multirow{3}{*}{Quantile Reg.} & MLP & +6.6 & +6.0 & +7.6 & -1.7 & +11.9 & +5.7 & -2.7 & +48.6 & +35.4 \\
 & RF & -1.5 & -1.0 & -3.3 & -9.9 & -7.7 & -7.3 & -7.7 & +15.7 & +19.9 \\
 & LR & -0.1 & +0.5 & -0.5 & +1.6 & +0.5 & +0.3 & +19.4 & +1.7 & +0.5 \\
\bottomrule
\end{tabular}%
}



==> tables/qis.tex <==
\begin{tabular}{l|lc}
\hline
\textbf{Dataset}                                        & \textbf{Selected quasi-identifiers}                                                                                                             & \textbf{\begin{tabular}[c]{@{}c@{}}\# Single-outs \\ per-seed range\end{tabular}} \\ \hline
COMPAS                                                  & Age, Race: Hispanic, Race: Other                                                                                                                & 5-13                                                                              \\
Covid                                                   & Age, Cerebro Vascular, Diabetes                                                                                                                 & 5-10                                                                              \\
Diabetes                                                & \begin{tabular}[c]{@{}l@{}}Time In Hospital, Race: African American, \\ Race: Other, Gender: Female, \\ Age: 70+, Age: {[}0-10{]}\end{tabular}  & 5-10                                                                              \\
Half Million                                            & Gender, State, Country                                                                                                                          & 180-216                                                                           \\
MIC                                                     & Age, Obesity, Chronic Pneumonia                                                                                                                 & 14-19                                                                             \\
Student Perf.                                           & School, Address, MJob, School Sup                                                                                                               & 4-12                                                                              \\
Surgery                                                 & \begin{tabular}[c]{@{}l@{}}Baseline Cancer, Baseline Dementia, \\ Baseline Digestive, Baseline OsteoArt, \\ Baseline Psych, Gender\end{tabular} & 4-10                                                                              \\ \hline
\end{tabular}

==> tables/qis2.tex <==
\begin{tabular}{l|lc}
\hline
\textbf{Dataset} & \textbf{Selected quasi-identifiers}                                                                                                             & \textbf{\begin{tabular}[c]{@{}c@{}}\# Single-outs \\ per-seed range\end{tabular}} \\ \hline
COMPAS           & Age, Race: Native American, AgeCat: 25-45                                                                                                                & 5-13                                                                              \\ \hline
Covid            & Age, Cerebro Vascular, Diabetes                                                                                                                 & 5-10                                                                              \\ \hline
Diabetes         & \begin{tabular}[c]{@{}l@{}}Time In Hospital, Race: African American, \\ Race: Other, Gender: Female, \\ Age: 70+, Age: {[}0-10{]}\end{tabular}  & 5-10                                                                              \\ \hline
Half Million     & Gender, State, Country                                                                                                                          & 180-216                                                                           \\ \hline
MIC              & Age, Obesity, Chronic Pneumonia                                                                                                                 & 14-19                                                                             \\ \hline
Student Perf.    & School, Address, MJob, School Sup                                                                                                               & 4-12                                                                              \\ \hline
Surgery          & \begin{tabular}[c]{@{}l@{}}Baseline Cancer, Baseline Dementia, \\ Baseline Digestive, Baseline OsteoArt, \\ Baseline Psych, Gender\end{tabular} & 4-10                                                                              \\ \hline
\end{tabular}

==> tables/ref_models_comparison.tex <==
\begin{tabular}{c|c|cccccc}
\hline
Dataset                                                                          & \begin{tabular}[c]{@{}c@{}}\# Ref. \\ Models\end{tabular} & \begin{tabular}[c]{@{}c@{}}Decision \\ Tree\end{tabular} & \begin{tabular}[c]{@{}c@{}}Logistic \\ Regression\end{tabular} & \begin{tabular}[c]{@{}c@{}}Naive \\ Bayes\end{tabular} & \begin{tabular}[c]{@{}c@{}}Random \\ Forest\end{tabular} & MLP        & XGBoost    \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}COMPAS \\ Recidivism\end{tabular}}    & 1                                                         & 74.2 ± 0.6                                               & 51.4 ± 0.7                                                     & 50.5 ± 0.8                                             & 59.0 ± 4.2                                               & 60.0 ± 5.8 & 68.3 ± 0.9 \\
                                                                                 & 5                                                         & 76.7 ± 1.1                                               & 52.2 ± 0.8                                                     & 50.9 ± 0.7                                             & 61.6 ± 5.0                                               & 61.3 ± 6.6 & 71.5 ± 1.1 \\
                                                                                 & 10                                                        & 77.2 ± 0.9                                               & 52.1 ± 0.8                                                     & 50.8 ± 0.6                                             & 62.2 ± 5.3                                               & 61.8 ± 6.3 & 72.0 ± 1.0 \\
                                                                                 & 30                                                        & 77.5 ± 0.9                                               & 52.0 ± 0.9                                                     & 50.8 ± 0.7                                             & 62.6 ± 5.3                                               & 62.0 ± 6.3 & 72.4 ± 1.0 \\ \hline
\multirow{4}{*}{COVID}                                                           & 1                                                         & 73.0 ± 1.4                                               & 56.4 ± 0.7                                                     & 52.8 ± 2.0                                             & 70.6 ± 3.4                                               & 54.1 ± 3.8 & 79.2 ± 1.5 \\
                                                                                 & 5                                                         & 76.0 ± 1.0                                               & 57.8 ± 1.1                                                     & 53.0 ± 1.8                                             & 75.9 ± 3.3                                               & 57.8 ± 4.1 & 81.9 ± 1.6 \\
                                                                                 & 10                                                        & 76.6 ± 0.9                                               & 58.1 ± 1.2                                                     & 52.8 ± 1.6                                             & 77.0 ± 3.6                                               & 58.3 ± 4.2 & 82.1 ± 1.6 \\
                                                                                 & 30                                                        & 77.1 ± 0.9                                               & 58.2 ± 1.6                                                     & 52.9 ± 1.7                                             & 77.5 ± 3.8                                               & 58.2 ± 4.3 & 82.5 ± 1.4 \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Diabetes \\ Readmission\end{tabular}} & 1                                                         & 73.6 ± 0.2                                               & 51.8 ± 0.2                                                     & 50.3 ± 0.1                                             & 76.3 ± 9.2                                               & 56.4 ± 6.4 & 60.9 ± 0.4 \\
                                                                                 & 5                                                         & 75.0 ± 0.2                                               & 52.1 ± 0.4                                                     & 50.4 ± 0.1                                             & 80.6 ± 9.0                                               & 57.0 ± 6.8 & 63.6 ± 0.5 \\
                                                                                 & 10                                                        & 75.7 ± 0.2                                               & 52.1 ± 0.4                                                     & 50.4 ± 0.1                                             & 81.3 ± 8.9                                               & 57.1 ± 6.8 & 64.0 ± 0.4 \\
                                                                                 & 30                                                        & 76.3 ± 0.2                                               & 52.2 ± 0.4                                                     & 50.5 ± 0.1                                             & 81.8 ± 8.8                                               & 57.1 ± 6.8 & 64.4 ± 0.4 \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Half \\ Million\end{tabular}}         & 1                                                         & 80.1 ± 0.3                                               & 54.9 ± 0.7                                                     & 53.0 ± 0.7                                             & 98.1 ± 0.4                                               & 53.6 ± 3.9 & 89.5 ± 0.2 \\
                                                                                 & 5                                                         & 82.9 ± 0.5                                               & 56.0 ± 0.5                                                     & 53.7 ± 0.3                                             & 99.1 ± 0.3                                               & 54.1 ± 3.7 & 91.9 ± 0.2 \\
                                                                                 & 10                                                        & 83.5 ± 0.4                                               & 56.2 ± 0.5                                                     & 53.7 ± 0.4                                             & 99.2 ± 0.2                                               & 54.1 ± 3.7 & 92.3 ± 0.2 \\
                                                                                 & 30                                                        & 84.1 ± 0.3                                               & 56.4 ± 0.4                                                     & 53.7 ± 0.5                                             & 99.2 ± 0.2                                               & 54.2 ± 3.8 & 92.6 ± 0.2 \\ \hline
\multirow{4}{*}{Locations}                                                       & 1                                                         & 77.2 ± 1.1                                               & 86.4 ± 0.8                                                     & 72.6 ± 1.6                                             & 96.7 ± 2.6                                               & 79.1 ± 1.0 & 87.2 ± 0.7 \\
                                                                                 & 5                                                         & 79.8 ± 0.7                                               & 89.6 ± 0.5                                                     & 74.2 ± 1.9                                             & 98.0 ± 1.8                                               & 77.9 ± 1.3 & 89.4 ± 0.8 \\
                                                                                 & 10                                                        & 80.3 ± 0.8                                               & 90.4 ± 0.4                                                     & 74.4 ± 1.8                                             & 98.2 ± 1.6                                               & 77.7 ± 1.5 & 89.9 ± 0.7 \\
                                                                                 & 30                                                        & 80.7 ± 0.8                                               & 90.7 ± 0.3                                                     & 74.8 ± 1.8                                             & 98.2 ± 1.6                                               & 77.6 ± 1.9 & 90.2 ± 0.8 \\ \hline
\multirow{4}{*}{Mammography}                                                     & 1                                                         & 52.2 ± 0.3                                               & 49.9 ± 0.7                                                     & 49.7 ± 1.1                                             & 57.5 ± 2.3                                               & 51.8 ± 0.6 & 53.4 ± 0.3 \\
                                                                                 & 5                                                         & 52.4 ± 0.2                                               & 49.9 ± 0.5                                                     & 49.9 ± 0.7                                             & 58.9 ± 2.8                                               & 51.7 ± 0.8 & 54.1 ± 0.6 \\
                                                                                 & 10                                                        & 52.6 ± 0.3                                               & 50.1 ± 0.7                                                     & 49.8 ± 0.8                                             & 59.3 ± 2.7                                               & 52.0 ± 0.8 & 54.2 ± 0.6 \\
                                                                                 & 30                                                        & 52.7 ± 0.1                                               & 50.3 ± 0.6                                                     & 49.8 ± 0.8                                             & 59.4 ± 2.9                                               & 51.9 ± 0.9 & 54.5 ± 0.8 \\ \hline
\multirow{4}{*}{MIC}                                                             & 1                                                         & 62.8 ± 1.2                                               & 62.6 ± 1.2                                                     & 56.0 ± 1.4                                             & 70.6 ± 5.2                                               & 59.1 ± 4.0 & 70.9 ± 2.2 \\
                                                                                 & 5                                                         & 64.1 ± 2.3                                               & 65.4 ± 1.3                                                     & 55.9 ± 1.2                                             & 74.5 ± 6.7                                               & 60.3 ± 2.8 & 72.5 ± 2.6 \\
                                                                                 & 10                                                        & 64.7 ± 2.7                                               & 65.5 ± 1.5                                                     & 55.8 ± 1.3                                             & 75.1 ± 7.1                                               & 60.6 ± 2.7 & 72.9 ± 2.5 \\
                                                                                 & 30                                                        & 65.2 ± 2.9                                               & 66.0 ± 1.8                                                     & 55.8 ± 1.3                                             & 75.5 ± 7.5                                               & 61.0 ± 3.1 & 72.9 ± 2.7 \\ \hline
\multirow{4}{*}{Purchases-10}                                                    & 1                                                         & 76.7 ± 0.4                                               & 65.0 ± 0.3                                                     & 53.1 ± 0.3                                             & 98.0 ± 0.8                                               & 62.6 ± 0.6 & 91.4 ± 0.2 \\
                                                                                 & 5                                                         & 79.2 ± 0.4                                               & 68.3 ± 0.4                                                     & 53.1 ± 0.2                                             & 99.1 ± 0.4                                               & 64.1 ± 1.7 & 94.2 ± 0.2 \\
                                                                                 & 10                                                        & 79.8 ± 0.3                                               & 69.0 ± 0.4                                                     & 52.9 ± 0.3                                             & 99.2 ± 0.4                                               & 64.3 ± 2.2 & 94.6 ± 0.1 \\
                                                                                 & 30                                                        & 80.4 ± 0.2                                               & 69.5 ± 0.2                                                     & 52.7 ± 0.4                                             & 99.3 ± 0.3                                               & 64.4 ± 2.6 & 94.9 ± 0.1 \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Student \\ Performance\end{tabular}}  & 1                                                         & 75.5 ± 1.0                                               & 61.8 ± 2.8                                                     & 53.7 ± 1.6                                             & 86.9 ± 5.0                                               & 80.7 ± 1.8 & 87.5 ± 1.5 \\
                                                                                 & 5                                                         & 77.6 ± 1.3                                               & 65.2 ± 2.3                                                     & 53.8 ± 2.0                                             & 89.5 ± 4.6                                               & 84.8 ± 1.2 & 91.3 ± 1.1 \\
                                                                                 & 10                                                        & 77.8 ± 1.4                                               & 65.7 ± 2.5                                                     & 54.0 ± 2.3                                             & 90.1 ± 4.0                                               & 84.8 ± 1.9 & 91.7 ± 1.6 \\
                                                                                 & 30                                                        & 78.4 ± 2.1                                               & 66.8 ± 2.8                                                     & 54.1 ± 2.0                                             & 90.6 ± 4.2                                               & 85.8 ± 1.4 & 92.6 ± 1.6 \\ \hline
\multirow{4}{*}{Surgery}                                                         & 1                                                         & 62.3 ± 0.4                                               & 51.5 ± 0.5                                                     & 50.2 ± 0.7                                             & 77.0 ± 2.5                                               & 64.3 ± 5.3 & 64.3 ± 0.7 \\
                                                                                 & 5                                                         & 64.4 ± 0.6                                               & 51.8 ± 0.4                                                     & 50.4 ± 0.6                                             & 81.6 ± 2.8                                               & 65.4 ± 5.2 & 67.1 ± 0.5 \\
                                                                                 & 10                                                        & 64.9 ± 0.5                                               & 51.7 ± 0.5                                                     & 50.6 ± 0.7                                             & 82.5 ± 2.8                                               & 65.7 ± 5.3 & 67.6 ± 0.5 \\
                                                                                 & 30                                                        & 65.0 ± 0.4                                               & 51.7 ± 0.4                                                     & 50.8 ± 0.8                                             & 83.2 ± 2.8                                               & 66.0 ± 5.4 & 67.9 ± 0.4 \\ \hline
\end{tabular}

==> tables/singleouts_catch.tex <==

\begin{tabular}{lcccc}
\toprule
Dataset & RF & XGB & MLP & SVM \\
\midrule
Adult  & \miacell{2}{4}{6}{3} & \miacell{3}{3}{5}{2} & \miacell{5}{4}{6}{4} & \miacell{2}{3}{4}{5} \\
Bank   & \miacell{4}{2}{5}{3} & \miacell{2}{5}{3}{4} & \miacell{6}{4}{5}{3} & \miacell{3}{2}{4}{6} \\
Credit & \miacell{1}{4}{2}{5} & \miacell{5}{3}{6}{4} & \miacell{2}{5}{4}{3} & \miacell{4}{6}{3}{5} \\
\bottomrule
\end{tabular}

==> tables/train_test.tex <==
\resizebox{\columnwidth}{!}{%
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{lcccccc}
\hline
               & \multicolumn{2}{c}{\textbf{COMPAS}}              & \multicolumn{2}{c}{\textbf{MIC}}                 & \multicolumn{2}{c}{\textbf{Surgery}}             \\ \cline{2-7} 
\textbf{Model} & \textbf{Train acc.} & \textbf{Test acc.}         & \textbf{Train acc.} & \textbf{Test acc.}         & \textbf{Train acc.} & \textbf{Test acc.}         \\ \hline
RF             & 0.715 $\pm$ 0.022   & \textbf{0.683 $\pm$ 0.009} & 0.905 $\pm$ 0.008   & 0.892 $\pm$ 0.004          & 0.940 $\pm$ 0.007   & 0.872 $\pm$ 0.003          \\
MLP            & 0.758 $\pm$ 0.064   & 0.659 $\pm$ 0.028          & 0.924 $\pm$ 0.039   & 0.862 $\pm$ 0.009          & 0.881 $\pm$ 0.059   & 0.711 $\pm$ 0.012          \\
NB             & 0.605 $\pm$ 0.021   & 0.598 $\pm$ 0.014          & 0.413 $\pm$ 0.032   & 0.333 $\pm$ 0.029          & 0.733 $\pm$ 0.004   & 0.732 $\pm$ 0.004          \\
DT             & 0.984 $\pm$ 0.001   & 0.561 $\pm$ 0.012          & 1.000 $\pm$ 0.000   & 0.820 $\pm$ 0.018          & 1.000 $\pm$ 0.000   & 0.811 $\pm$ 0.004          \\
XGB            & 0.823 $\pm$ 0.006   & 0.659 $\pm$ 0.008          & 1.000 $\pm$ 0.000   & \textbf{0.894 $\pm$ 0.005} & 0.942 $\pm$ 0.003   & \textbf{0.880 $\pm$ 0.002} \\
LR             & 0.684 $\pm$ 0.005   & 0.678 $\pm$ 0.010          & 0.970 $\pm$ 0.015   & 0.862 $\pm$ 0.009          & 0.753 $\pm$ 0.003   & 0.750 $\pm$ 0.005          \\ \hline
\end{tabular}%
}


==> tables/wilcoxon.tex <==
\resizebox{\columnwidth}{!}{%
\begin{tabular}{clllll}
\multicolumn{1}{c|}{\multirow{2}{*}{Num Ref.}} & \multicolumn{1}{c|}{\multirow{2}{*}{Dataset}} & \multicolumn{2}{c|}{Attack-P}                              & \multicolumn{2}{c}{QMIA}                              \\ \cline{3-6} 
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c}{Statistic} & \multicolumn{1}{c|}{p}     & \multicolumn{1}{c}{Statistic} & \multicolumn{1}{c}{p} \\ \hline
\multicolumn{1}{c|}{1}                         & \multicolumn{1}{l|}{COMPAS}                   & 0.0                           & \multicolumn{1}{l|}{0.006} & 14.0                          & 0.387                 \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{l|}{MIC}                      & 19.0                          & \multicolumn{1}{l|}{0.863} & 27.0                          & 1.000                 \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{l|}{Surgery}                  & 27.0                          & \multicolumn{1}{l|}{1.000} & 6.0                           & 0.082                 \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{5}}        & \multicolumn{1}{l|}{COMPAS}                   & 0.0                           & \multicolumn{1}{l|}{0.006} & 4.0                           & 0.041                 \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{l|}{MIC}                      & 21.0                          & \multicolumn{1}{l|}{0.557} & 16.0                          & 0.551                 \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{l|}{Surgery}                  & 0.0                           & \multicolumn{1}{l|}{0.006} & 17.0                          & 0.551                 \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{10}}       & \multicolumn{1}{l|}{COMPAS}                   & 0.0                           & \multicolumn{1}{l|}{0.006} & 4.0                           & 0.041                 \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{l|}{MIC}                      & 18.0                          & \multicolumn{1}{l|}{0.375} & 16.0                          & 0.551                 \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{l|}{Surgery}                  & 0.0                           & \multicolumn{1}{l|}{0.006} & 20.0                          & 0.551                 \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{30}}       & \multicolumn{1}{l|}{COMPAS}                   & 0.0                           & \multicolumn{1}{l|}{0.006} & 5.0                           & 0.059                 \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{l|}{MIC}                      & 17.0                          & \multicolumn{1}{l|}{0.322} & 14.0                          & 0.387                 \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{l|}{Surgery}                  & 0.0                           & \multicolumn{1}{l|}{0.006} & 22.0                          & 0.625                 \\  
\end{tabular}%
}
